Generating Bindings in MPICH

The MPI Forum has recently adopted a Python scripting engine for generating the API text in the standard document. As a by-product, it made available reliable and rich descriptions of all MPI functions that are suited for scripting tools. Using these extracted API information, we developed a Python code generation toolbox to generate the language binding layers in MPICH. The toolbox replaces nearly 70,000 lines of manually maintained C and Fortran 2008 binding code with around 5,000 lines of Python scripts plus some simple configuration. In addition to completely eliminating code duplication in the binding layer and avoiding bugs from manual code copying , the code generation also minimizes the effort for API extension and code instrumentation. This is demonstrated in our implementation of MPI-4 large count functions and the prototyping of a next generation MPI profiling interface, QMPI.

==> Makefile <==
MAIN = python_binding
FIGS = figures
BIB = bib
TEX = text

TARGETS: $(MAIN).pdf
.PHONY: all clean

tex_files = $(shell find $(TEX) -name '*.tex' -print)
bib_files = $(shell find $(BIB) -name '*.bib' -print)
fig_files = $(shell find $(FIGS) \
		\( -name '*.eps' -print \) -or \( -name '*.epsi' -print \) \
		-or \( -name '*.ps' -print \) -or \( -name '*.png' -print \) \
		-or \( -name '*.fig' -print \) -or \( -name '*.pdf' -print \) \
		-or \( -name '*.data' -print \) -or \( -name '*.plt' -print \) \
	)

$(MAIN).pdf: $(MAIN).tex $(tex_files) $(bib_files) $(fig_files)
	@if test "`which rubber`" != "" ; then \
		TEXMFOUTPUT=`pwd` rubber -d $(MAIN) ; \
	else \
		pdflatex $(MAIN) | tee latex.out ; \
		if grep -q '^LaTeX Warning: Citation.*undefined' latex.out; then \
			bibtex $(MAIN); \
			touch .rebuild; \
		fi ; \
		while [ -f .rebuild -o \
			-n "`grep '^LaTeX Warning:.*Rerun' latex.out`" ]; do \
			rm -f .rebuild; \
			pdflatex $(MAIN) | tee latex.out; \
		done ; \
		rm -f latex.out ; \
	fi

$(MAIN)-embedfonts.pdf: $(MAIN).pdf
	gs -o $@ -sDEVICE=pdfwrite -dEmbedAllFonts=true -dCompatibilityLevel=1.5 -dSettings=/printer  $^

clean:
	@if test "`which rubber`" != "" ; then \
		rubber -d --clean $(MAIN) && rm -f comment.cut; \
	else \
		find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
			\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
			\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
			\( -name '*.toc' -print \) | xargs rm -f; \
		rm -f $(MAIN).dvi $(MAIN).log $(MAIN).ps $(MAIN).pdf $(MAIN).out \
			_region_* TAGS ; \
	fi

